RIS-Assisted Cell-Free Massive MIMO Relying on Reflection Pattern Modulation

We propose reflection pattern modulation-aided reconfigurable intelligent surface (RPM-RIS)-assisted cell-free massive multiple-input-multiple-output (CF-mMIMO) schemes for green uplink transmission. In our RPM-RIS-assisted CF-mMIMO system, extra information is conveyed by the indices of the active RIS blocks, exploiting the joint benefits of both RIS-assisted CF-mMIMO transmission and RPM. Since only part of the RIS blocks are active, our proposed architecture strikes a flexible energy \emph{vs.} spectral efficiency (SE) trade-off. We commence with introducing the system model by considering spatially correlated channels. Moreover, we conceive a channel estimation scheme subject to the linear minimum mean-square error (MMSE) constraint, yielding sufficient information for the subsequent signal processing steps. Then, upon exploiting a so-called large-scale fading decoding (LSFD) scheme, the uplink signal-to-interference-and-noise ratio (SINR) is derived based on the RIS ON/OFF statistics, where both maximum ratio (MR) and local minimum mean-square error (L-MMSE) combiners are considered. By invoking the MR combiner, the closed-form expression of the uplink SE is formulated based only on the channel statistics. Furthermore, we derive the total energy efficiency (EE) of our proposed RPM-RIS-assisted CF-mMIMO system. Additionally, we propose a chaotic sequence-based adaptive particle swarm optimization (CSA-PSO) algorithm to maximize the total EE by designing the RIS phase shifts. Finally, our simulation results demonstrate that the proposed RPM-RIS-assisted CF-mMIMO architecture strikes an attractive SE \emph{vs.} EE trade-off, while the CSA-PSO algorithm is capable of attaining a significant EE performance gain compared to conventional solutions.

==> acronyms.tex <==
%
%acronyms

\newacronym{AWGN}{AWGN}{additive white Gaussian noise}

\newacronym{BABF}{BABF}{blind adaptive beamforming}

\newacronym{BER}{BER}{bit error ratio}

\newacronym{CW}{CW}{continuous wave}

\newacronym{CU}{CU}{control unit}

\newacronym{JML}{JML}{joint maximum-likelihood}

\newacronym{DPSK}{DPSK}{differential phase shift key}

\newacronym{PSK}{PSK}{phase shift key}

\newacronym{EM}{EM}{expectation maximization}

\newacronym{PDF}{PDF}{probability density function}

\newacronym{CSI}{CSI}{channel state information}

\newacronym{EPC}{EPC}{electronic product code}

\newacronym{RF}{RF}{radio frequency}

\newacronym{RIP}{RIP}{rotational invariance property}

\newacronym{RFID}{RFID}{radio frequency identification}

\newacronym{IC}{IC}{integrated circuit}

\newacronym{IoTs}{IoTs}{Internet of Things}

\newacronym{ULA}{ULA}{uniform linear array}

\newacronym{UHF}{UHF}{ultra high frequency}

\newacronym{OLS}{OLS}{ordinary least square}

\newacronym{QCQPs}{QCQPs}{quadratically constrained quadratic programs}

\newacronym{SDR}{SDR}{semidefinite relaxation}

\newacronym{SCA}{SCA}{successive convex approximation}

\newacronym{WET}{WET}{wireless energy transfer}

\newacronym{UWB}{UWB}{ultrawide bandwidth}

\newacronym{ToA}{ToA}{time-of-arrival}

\newacronym{PoA}{PoA}{phase-of-arrival}

\newacronym{DoA}{DoA}{direction-of-arrival}

\newacronym{RSS}{RSS}{received signal strength}

\newacronym{MSE}{MSE}{mean square error}

\newacronym{DoF}{DoF}{degree of freedom}

\newacronym{UAV}{UAV}{unmanned aerial vehicle}

\newacronym{CAMs}{CAMs}{cooperative awareness messages}

\newacronym{BS}{BS}{base station}

\newacronym{ID}{ID}{identification}

\newacronym{PL}{PL}{platoon leader}

\newacronym{PM}{PM}{platoon member}
\newacronym{PMs}{PMs}{platoon members}

\newacronym{a.k.a.}{a.k.a.}{also know as}

\newacronym{DPM}{DPM}{disconnected platoon member}

\newacronym{BaS}{BaS}{Braking and Stopping}

\newacronym{TAs}{TAs}{transmit antennas}

\newacronym{RAs}{RAs}{receive antennas}

\newacronym{3D}{3D}{three-dimensional}

\newacronym{ACK}{ACK}{acknowledgement}

\newacronym{V2V}{V2V}{vehicle-to-vehicle}

\newacronym{V2I}{V2I}{vehicle-to-infrastructure}

\newacronym{WLAN}{WLAN}{wireless local area network}

\newacronym{UAVs}{UAVs}{unmanned aerial vehicles}

\newacronym{ML}{ML}{machine learning}

\newacronym{TOA}{TOA}{time of arrival}

\newacronym{UWB}{UWB}{ultrawideband}

\newacronym{OBU}{OBU}{on-board unit}

\newacronym{LOS}{LOS}{line-of-sight}

\newacronym{RIB}{RIB}{rotational invariance beamforming}




















